Synthetic Alone: Exploring the Dark Side of Synthetic Data for Grammatical Error Correction

Data-centric AI approach aims to enhance the model performance without modifying the model and has been shown to impact model performance positively. While recent attention has been given to data-centric AI based on synthetic data, due to its potential for performance improvement, data-centric AI has long been exclusively validated using real-world data and publicly available benchmark datasets. In respect of this, data-centric AI still highly depends on real-world data, and the verification of models using synthetic data has not yet been thoroughly carried out. Given the challenges above, we ask the question: Does data quality control (noise injection and balanced data), a data-centric AI methodology acclaimed to have a positive impact, exhibit the same positive impact in models trained solely with synthetic data? To address this question, we conducted comparative analyses between models trained on synthetic and real-world data based on grammatical error correction (GEC) task. Our experimental results reveal that the data quality control method has a positive impact on models trained with real-world data, as previously reported in existing studies, while a negative impact is observed in models trained solely on synthetic data.

==> tables/results_1.tex <==
% \begin{table*}[ht!]
%   \centering
%   \setlength\tabcolsep{3.8pt}
% \resizebox{0.85\textwidth}{!}{
%   \begin{tabular}{lccccc} 
%     \toprule
%         \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Dev.}} & \multicolumn{2}{c}{\textbf{Test}} & \multirow{2}{*}{\textbf{Avg. Imp.}} \\
%     \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%          & Ign F1 & F1 & Ign F1 & F1 \\
%     \midrule
%         \midrule
%         \multicolumn{6}{c}{\textit{Baselines}} \\
%         \midrule
%         $\text{BERT-multilingual}$ \cite{devlin2019bert} & 55.54 & 55.45 & 52.72 & 52.59 & - \\ 
%         \cdashline{1-6}[0.8pt/1.2pt]
%         $\text{KoBERT}$ (\href{https://github.com/SKTBrain/KoBERT}{SKT Brain, 2019})  & 41.87 & 40.23 & 38.25 & 38.18 & -\\
%         $\text{KLUE-BERT}$ \cite{park2021klue} & 60.19 & 60.11 & 59.91 & 59.80 & - \\
%         $\text{KLUE-RoBERTa}$ \cite{park2021klue} & 62.41 & 62.27 & 59.67 & 59.44 & - \\
        

%     \midrule
%     \multicolumn{6}{c}{\textit{Our Models}} \\
%     \midrule
%         TREKER$_{\text{BERT-multilingual}}$ & 56.41 (+0.87) & 66.34 (+10.89) & 55.32 (+2.60) & 57.92 (+5.33) & +4.92\\
%         \cdashline{1-6}[0.8pt/1.2pt]
%         TREKER$_{\text{KoBERT}}$  & 49.64 (+7.77) & 51.20 (+10.97) & 47.52 (+9.27) & 49.49 (+11.31) & +9.83\\
%         TREKER$_{\text{KLUE-BERT}}$ & 61.17 (+0.98) & 68.71 (+8.60) & \textbf{60.73} (+0.82) & 61.62 (+1.82) & +3.06\\
%         TREKER$_{\text{KLUE-RoBERTa}}$ & \textbf{63.43} (+1.02)& \textbf{69.78} (+7.51) & 59.70 (+0.03) & \textbf{62.63} (+3.19) & +2.94 \\
%     \bottomrule
%   \end{tabular}
% }
%   \caption{RE results ($\%$) of different RE models on \texttt{\textbf{TREK}} dataset. 
%   Ign F1 refers to the F1 score excluding the relation instances mentioned in the train set. Dev. and Avg. Imp. indicate the development set and the average of performance improvement between baselines and ours from both Ign F1 and F1, respectively.
% }
%   \label{tab:TED_AIHUB_result}
% \end{table*}




\begin{table}[t]
{\tiny
  \centering
  \setlength\tabcolsep{3.8pt}
\resizebox{\columnwidth}{!}{
  \begin{tabular}{lcccc} 
    \toprule
        \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{AI-HUB}} & \multicolumn{2}{c}{\textbf{TED}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
         & Dev & Test & Dev & Test \\
    \midrule
        \midrule
        \multicolumn{5}{c}{\textit{Baseline}} \\
        \midrule
        $\text{Clean}$ & \textbf{67.95} & \textbf{65.69} & \textbf{59.41} & \textbf{56.14}  \\ 
        % $\text{KoBERT}$ (\href{https://github.com/SKTBrain/KoBERT}{SKT Brain, 2019})  & 41.87 & 40.23 & 38.25 & 38.18 \\
        % $\text{KLUE-BERT}$ \cite{park2021klue} & 60.19 & 60.11 & 59.91 & 59.80 \\
        % $\text{KLUE-RoBERTa}$ \cite{park2021klue} & 62.41 & 62.27 & 59.67 & 59.44 \\
        

    \midrule
    \multicolumn{5}{c}{\textit{Noised-X}} \\
    \midrule
        \textit{Noised-0.1} & 65.67 & 63.82 & 58.07 & 55.43\\
        \textbf{\texttt{Noised-0.2}} & 66.52 & 64.66 & 58.97 & 56.55\\
        \texttt{Noised-0.4} & 67.11 & 65.37 & 58.60 & 55.57\\
        Noised-0.6 & 65.99 & 63.90 & 57.74 & 54.69\\
        Noised-0.8 & 65.80 & 64.08 & 57.54 & 54.20\\
        Noised-1.0 & 67.27 & 64.65 & 58.09 & 55.20\\
        
% \textbf{\texttt{TREKER}}$_{\text{KoBERT}}$ \\
    \bottomrule
  \end{tabular}
}
  \caption{Experimental results of synthetic data based on BTS. AIHUB and TED are compared with the baseline at various ratios of noise insertion, respectively.
}
  \label{tab:TED_AIHUB_result}}
\end{table}

==> tables/results_2.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% \begin{table}[t]
%   \centering
% \begin{tabular}{@{}clrr@{}}
% \toprule
% \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Mixed ratio\\ (clean:noise)\end{tabular}} & Noised-X & \multicolumn{1}{c}{Dev.}  & \multicolumn{1}{c}{Test} \\ \midrule
% \multirow{2}{*}{5:5}                                                                    & Noised-0.4      & 68.97                     & 66.58                    \\
%                                                                                         & 1.0      & 67.35                     & 64.95                    \\ \midrule
% \multirow{2}{*}{4:6}                                                                    & 0.4      & 68.87                     & 66.6                     \\
%                                                                                         & 1.0      & 66.71                     & 64.98                    \\ \midrule
% \multirow{2}{*}{3:7}                                                                    & 0.4      & 68.93                     & 66.8                     \\
%                                                                                         & 1.0      & 65.33                     & 63.2                     \\ \midrule
% \multirow{2}{*}{2:8}                                                                    & 0.4      & 68.45                     & 67.04                    \\
%                                                                                         & 1.0      & 62.20                     & 59.72                    \\ \midrule
% \multirow{2}{*}{1:9}                                                                    & 0.4      & 68.46                     & 66.25                    \\
%                                                                                         & 1.0      & \multicolumn{1}{l}{xx.xx} & 53.16                    \\  \midrule 
% \end{tabular}
% \caption{Mixed ratio AIHUB}
% \label{tab:Mixed_AIHUB}
% \end{table}








%%%%%%%%%%%%%%%%%%%%5TED 

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% \begin{table}[t]
%   \centering
% \begin{tabular}{@{}cllr@{}}
% \toprule
% \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Mixed ratio\\ (clean:noise)\end{tabular}} & Noised-X & \multicolumn{1}{c}{Dev.} & \multicolumn{1}{c}{Test} \\ \midrule
% \multirow{2}{*}{5:5}                                                                    & 0.2      & xx.xx                   & 56.94                    \\
%                                                                                         & 1.0      & xx.xx                   & 55.48                    \\ \midrule
% \multirow{2}{*}{4:6}                                                                    & 0.2      & xx.xx                   & 57.39                    \\
%                                                                                         & 1.0      & xx.xx                   & 53.33                    \\ \midrule
% \multirow{2}{*}{3:7}                                                                    & 0.2      & xx.xx                   & 56.86                    \\
%                                                                                         & 1.0      & xx.xx                   & 51.58                    \\ \midrule
% \multirow{2}{*}{2:8}                                                                    & 0.2      & xx.xx                   & 56.91                    \\
%                                                                                         & 1.0      & xx.xx                   & 46.70                    \\ \midrule
% \multirow{2}{*}{1:9}                                                                    & 0.2      & xx.xx                   & 57.21                    \\
%                                                                                         & 1.0      & xx.xx                   & 38.15                    \\ \midrule 
% \end{tabular}
% \caption{Mixed ratio}
% \label{tab:Mixed_TED}
% \end{table}



\begin{table}[t]
{\tiny
  \centering
  \resizebox{\linewidth}{!}{
\begin{tabular}{@{}cllr@{}}
\toprule
\multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}\textbf{Mixed ratio}\\ (clean:noise)\end{tabular}} & \textbf{Noised-X} & \multicolumn{1}{c}{\textbf{AI-HUB}} & \multicolumn{1}{c}{\textbf{TED}} \\ \midrule\midrule

\multirow{2}{*}{5:5}                                                                    & Noised-best      & 66.58                   & 56.94                    \\
                                                                                        & Noised-1.0      & 64.95                   & 55.48                    \\ \midrule
\multirow{2}{*}{4:6}                                                                    & Noised-best       & 66.60                   & 57.39                    \\
                                                                                        & Noised-1.0      & 64.98                   & 53.33                    \\ \midrule
\multirow{2}{*}{3:7}                                                                    & Noised-best       & 66.80                   & 56.86                    \\
                                                                                        & Noised-1.0      & 63.20                   & 51.58                    \\ \midrule
\multirow{2}{*}{2:8}                                                                    & Noised-best       & 67.04                   & 56.91                    \\
                                                                                        & Noised-1.0      & 59.72                   & 46.70                    \\ \midrule
\multirow{2}{*}{1:9}                                                                    & Noised-best       & 66.25                   & 57.21                    \\
                                                                                        & Noised-1.0      & 53.16                   & 38.15                    \\ 
                                                                                        \bottomrule
\end{tabular}}
\caption{Mixed ratio results}
\label{tab:Mixed_results}}
\end{table}

==> tables/results_3.tex <==
\begin{table}[t]
{\tiny
  \centering
  \setlength\tabcolsep{3.8pt}
\resizebox{\columnwidth}{!}{
  \begin{tabular}{lcccc} 
    \toprule
        \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{AI-HUB}} & \multicolumn{2}{c}{\textbf{TED}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
         & Dev & Test & Dev & Test \\
    \midrule
        \midrule
        \multicolumn{5}{c}{\textit{Baseline}} \\
        \midrule
        $\text{Clean}$ & \textbf{67.95} & \textbf{65.69} & \textbf{59.41} & \textbf{56.14}  \\ 
        

    \midrule
    \multicolumn{5}{c}{\textit{Noised-X}} \\
    \midrule
        \textit{Noised-0.1} & 65.67 & 63.82 & 58.07 & 55.43\\
        \textbf{\texttt{Noised-0.2}} & 66.52 & 64.66 & 58.97 & 56.55\\
        \texttt{Noised-0.4} & 67.11 & 65.37 & 58.60 & 55.57\\
        Noised-0.6 & 65.99 & 63.90 & 57.74 & 54.69\\
        Noised-0.8 & 65.80 & 64.08 & 57.54 & 54.20\\
        Noised-1.0 & 67.27 & 64.65 & 58.09 & 55.20\\
        
% \textbf{\texttt{TREKER}}$_{\text{KoBERT}}$ \\
    \bottomrule
  \end{tabular}
}
  \caption{Baseline has not undergone any processing on the data, and Noised-X trained on synthetic data. Dev. indicates the development set. 
}
  \label{tab:TED_AIHUB_result}}
\end{table}
